A Unified Framework for Event-based Frame Interpolation with Ad-hoc Deblurring in the Wild

Effective video frame interpolation hinges on the adept handling of motion in the input scene. Prior work acknowledges asynchronous event information for this, but often overlooks whether motion induces blur in the video, limiting its scope to sharp frame interpolation. We instead propose a unified framework for event-based frame interpolation that performs deblurring ad-hoc and thus works both on sharp and blurry input videos. Our model consists in a bidirectional recurrent network that incorporates the temporal dimension of interpolation and fuses information from the input frames and the events adaptively based on their temporal proximity. To enhance the generalization from synthetic data to real event cameras, we integrate self-supervised framework with the proposed model to enhance the generalization on real-world datasets in the wild. At the dataset level, we introduce a novel real-world high-resolution dataset with events and color videos named HighREV, which provides a challenging evaluation setting for the examined task. Extensive experiments show that our network consistently outperforms previous state-of-the-art methods on frame interpolation, single image deblurring, and the joint task of both. Experiments on domain transfer reveal that self-supervised training effectively mitigates the performance degradation observed when transitioning from synthetic data to real-world data. Code and datasets are available at https://github.com/AHupuJR/REFID.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/ablation_study.tex <==
\subsection{Ablation study}
%
% Table 3:
% - The 
%
%
% Table 4:
% - 
%
%
\vspace{-3mm}
\input{tables/ablation_studies}
All the ablation studies are conducted with self-supervised training from scratch on each dataset.

\textbf{Ablation on Losses: }
Table~\ref{table:ablation_loss} shows the distinct contributions of different loss components — brightness increment loss, blur consistency loss, and warp loss — to the performance of our image deblurring model, and reports PSNR and SSIM on GoPro and HighREV.
The blur consistency loss appears critical for achieving decent performance, as reflected by the results where this loss was excluded (i.e., the combination of brightness increment loss and warp loss). The model performance dropped dramatically on both datasets, reaching a PSNR of only 7.22 dB and 10.26 dB on GoPro and HighREV respectively, with correspondingly low SSIM values.
On the other hand, the inclusion of the warp loss is highly beneficial. For instance, when this loss was added to the blur consistency loss, the PSNR on the HighREV dataset increased substantially from 23.41 dB to 28.53 dB, with similar improvements on the synthetic GoPro dataset.
The addition of the brightness increment loss to the blur loss led to only minor improvements on the synthetic GoPro but substantially benefits the real-world results on the HighREV dataset where the PSNR increases from 23.41 dB to 27.81 dB. This difference in performance boost could stem from the fact that the events in the GoPro dataset are generated with interpolated frames that often yield subtle artifacts that affect synthetic event generation.
Finally, it's worth noting that the combination of all three losses yielded the best results. The model achieved a PSNR of 28.88 dB on GoPro and 30.04 dB on HighREV, with high SSIM values, demonstrating the complementary roles of these loss components.
This finding reinforces the effectiveness of our proposed framework that capitalizes on the different constraints offered by each of these losses in the image deblurring process.
%\begin{figure}
%    \centering
%    \includegraphics[width=0.98\textwidth]{figures/ablation.pdf}
%    \caption{\textbf{Visualized examples for ablation study.}}
%    \label{fig:ablation}
%\end{figure}

\textbf{Ablation on Components:} Next we investigate the use of images of warped events at the input of our method, and the use of RobustNorm+, a voxel normalization method that deviates slightly from the RobustNorm in~\cite{stoffregen2020reducing}. 
Both normalize non-zero values as,
\begin{equation}
    \bar{\mathbf{V}}^{\text{RN}}_i(\textbf{x}) = \text{clip}\left(\frac{\mathbf{V}_i(\textbf{x}) - \textbf{V}_{i,1}}{\textbf{V}_{i,99} - \textbf{V}_{i,1}}, 0, 1\right)\quad    \bar{\mathbf{V}}^{\text{RN+}}_i(\textbf{x}) = \text{clip}\left(\frac{\mathbf{V}_i(\textbf{x})}{\textbf{V}_{i,99}}, 0, 1\right)
\end{equation}
where $\textbf{V}_{i,p}$ denotes the $p^\text{th}$ percentile of $\mathbf{V}_i(\textbf{x})$. We found that RobustNorm+ was more stable during training and lead to fewer outliers on samples with few events. We report an ablation of these components in Table~\ref{table:ablation_module}. Removing IWE from the input led to a 0.19 dB reduction on GoPro, and a 0.90 dB reduction on HighREV, justifying its use. We argue that the IWE is essential since it provides a sharp template for the network for placing edges at the output. We also find that RobustNorm+ increases the PSNR by 0.89 dB on GoPro and 1.69 dB on HighREV. %We found that this increase came especially from more stable training.



% \begin{table}[tb]
% % \captionsetup{font=small}
% % \vspace{-3mm}
% \caption{\small \textbf{Ablation on components.}}
% % \vspace{-3mm}
% \centering
% \small
% % \tiny
% \resizebox{0.95\textwidth}{!}{
% \setlength{\tabcolsep}{10pt}     % adjust the width of cell
% \renewcommand\arraystretch{1.0} % adjust hight of the row
% \begin{tabular}{ c  c  c || c   c  |  c  c }
% \bottomrule[0.15em]
% \rowcolor{tableHeadGray}
% & &  & \multicolumn{2}{c|}{GoPro} & \multicolumn{2}{c}{HighREV} \\
% \cline{4-7}
% \rowcolor{tableHeadGray}
% \multirow{-2}{*}{IWE} & \multirow{-2}{*}{Feat warp} & \multirow{-2}{*}{Our Norm} & PSNR & SSIM & PSNR & SSIM \\ \hline \hline
% \cmark & \xmark & \xmark & psnr & ssim & psnr & ssim \\
% \xmark & \cmark & \xmark & psnr & ssim & psnr & ssim \\
% \xmark & \xmark & \cmark & psnr & ssim & psnr & ssim \\ \hline
% \cmark & \cmark & \xmark & 23.78 & 0.831 & psnr & ssim \\
% \cmark & \xmark & \cmark & 7.22 & 0.0257? & psnr & ssim \\
% \xmark & \cmark & \cmark & psnr & ssim & psnr & ssim \\ \hline
% \cmark & \cmark & \cmark & 28.88 & 0.912 & 30.04 & 0.931 \\
% \bottomrule
% \hline
% \end{tabular}
% }
% \label{table:ablation_module}
% \vspace{-0.5cm}
% \end{table}



==> tables/ablation_studies.tex <==
\begin{minipage}[t]{0.49\linewidth}
% \captionsetup{font=small}
\captionof{table}{\small \textbf{Ablation on losses.} Brightness increment ($\mathcal{L}_\text{br. inc.}$), blur consistency ($\mathcal{L}_\text{blur cons.}$), and warping loss ($\mathcal{L}_\text{warp}$).}
% \vspace{-3mm}
\centering
\small
% \tiny
\resizebox{\textwidth}{!}{
%\setlength{\tabcolsep}{10pt}     % adjust the width of cell
%\renewcommand\arraystretch{1.0} % adjust hight of the row
\begin{tabular}{ c  c  c || c   c  |  c  c }
\bottomrule[0.15em]
\rowcolor{tableHeadGray}
& &  & \multicolumn{2}{c|}{GoPro} & \multicolumn{2}{c}{HighREV} \\
%\cline{4-7}
\rowcolor{tableHeadGray}
\multirow{-2}{*}{$\mathcal{L}_\text{br. inc.}$} & \multirow{-2}{*}{$\mathcal{L}_\text{blur cons.}$} & \multirow{-2}{*}{$\mathcal{L}_\text{warp}$} & PSNR & SSIM & PSNR & SSIM \\ \hline \hline
%\cmark & \xmark & \xmark & 6.84 & 0.044 & 9.425 & 0.131 \\
\xmark & \cmark & \xmark & 23.52 & 0.824 & 23.41 & 0.817 \\\hline
%\xmark & \xmark & \cmark & 6.38 & 0.056 & 9.77 & 0.130 \\ \hline
\cmark & \cmark & \xmark & 23.78 & 0.831 & 27.81 & 0.925 \\
\cmark & \xmark & \cmark & 7.22 & 0.026 & 10.26 & 0.175 \\
\xmark & \cmark & \cmark & 27.72 & 0.893 & 28.53 & 0.927 \\ \hline
\cmark & \cmark & \cmark & 28.88 & 0.912 & 30.04 & 0.931 \\
\bottomrule
\hline
\end{tabular}
}
\label{table:ablation_loss}
%\vspace{-0.5cm}
\end{minipage}
\begin{minipage}[t]{0.49\linewidth}
% \captionsetup{font=small}
\captionof{table}{\small \textbf{Ablation on components.} IWE: Using image of warped events for training. Voxel Norm: the method used for voxel normalization.}
% \vspace{-3mm}
\centering
\small
% \tiny
\resizebox{\textwidth}{!}{
%\setlength{\tabcolsep}{10pt}     % adjust the width of cell
\renewcommand\arraystretch{1.21} % adjust hight of the row
\begin{tabular}{ c  c || c   c  |  c  c }
\bottomrule[0.15em]
\rowcolor{tableHeadGray}
&  & \multicolumn{2}{c|}{GoPro} & \multicolumn{2}{c}{HighREV} \\
%\cline{4-7}
\rowcolor{tableHeadGray}
\multirow{-2}{*}{IWE} & \multirow{-2}{*}{Voxel Norm} & PSNR & SSIM & PSNR & SSIM \\ \hline \hline
\xmark & RobustNorm~\cite{Stoffregen19cvpr} & 27.95 & 0.896 & 28.98 & 0.894 \\
\cmark & RobustNorm~\cite{Stoffregen19cvpr} & 27.99 & 0.895 & 29.25 & 0.924 \\ 
\xmark & RobustNorm+ (Ours)                               & 28.59 & 0.909 & 30.04 & 0.931 \\\hline
\cmark & RobustNorm+ (Ours)                               & \textbf{28.88} & \textbf{0.912} & \textbf{30.94} & \textbf{0.937} \\
\bottomrule
\hline
\end{tabular}
}
\label{table:ablation_module}
\end{minipage}


==> tables/gopro_highrev_results.tex <==
\begin{table}
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{20pt}     % adjust the width of cell
\parbox{0.45\linewidth}{
\caption{\small \textbf{Comparison of motion deblurring methods on the GoPro dataset~\cite{nah2017deep}.} SRN+ and HINet+ denote event-enhanced versions of SRN~\cite{tao2018scale} and HINet~\cite{chen2021hinet}.}
% \vspace{-3mm}
\centering
\small
% \tiny
\resizebox{0.45\textwidth}{!}{
%\setlength{\tabcolsep}{30pt}     % adjust the width of cell
\renewcommand\arraystretch{1.0} % adjust hight of the row
\begin{tabular}{ l  || c | c |  c  |  c  }
\bottomrule[0.15em]
\rowcolor{tableHeadGray}
 Method &  Self-Sup.  &Events & PSNR $\uparrow$ & SSIM $\uparrow$  \\ \hline \hline
EDI~\cite{edi_pan}                  &\cmark&\cmark& 27.34 & 0.901 \\
Nah \etal \cite{nah2017deep}        &\xmark&\xmark& 29.08 & 0.914 \\
SRN~\cite{tao2018scale}             &\xmark&\xmark& 30.26 & 0.934 \\
SRN+~\cite{tao2018scale}            &\xmark&\cmark& 31.02 & 0.936 \\
D$^{2}$Nets~\cite{shang2021bringing}&\xmark&\cmark& 31.60 & 0.940 \\
LEMD~\cite{jiang2020}               &\xmark&\cmark& 31.79 & 0.949 \\
HINet~\cite{chen2021hinet}          &\xmark&\xmark& 32.71 & 0.959 \\
Restormer~\cite{Zamir2021Restormer} &\xmark&\xmark& 32.92 & 0.961 \\
ERDNet~\cite{haoyu2020learning}     &\xmark&\cmark& 32.99 & 0.935 \\
HINet+~\cite{chen2021hinet}         &\xmark&\cmark& 33.69 & 0.961 \\
EFNet~\cite{sun2022event}           &\xmark&\cmark& 35.46 & 0.972 \\
REFID~\cite{sun2023event}           &\xmark&\cmark& \textbf{35.91} & \textbf{0.973}\\ \hline \textbf{Ours}                &\cmark&\cmark& 28.88 & 0.912 \\
\textbf{Ours}                       &\xmark&\cmark& 35.52 & 0.972 \\
\bottomrule
\hline
\end{tabular}
}
\label{table:gopro}
% \vspace{-0.5cm}
}
\parbox{0.45\linewidth}{
\caption{\small \textbf{Comparison of event-based motion deblurring methods on the HighREV dataset~\cite{sun2023event}.} SRN+ and HINet+ denote event-enhanced versions of SRN~\cite{tao2018scale} and HINet~\cite{chen2021hinet}. Draft}
% \vspace{-3mm}
\centering
\small
% \tiny
\resizebox{0.45\textwidth}{!}{
%\setlength{\tabcolsep}{20pt}     % adjust the width of cell
\renewcommand\arraystretch{1.0} % adjust hight of the row
\begin{tabular}{ l  || c |  c  |  c |  c }
\bottomrule[0.15em]
\rowcolor{tableHeadGray}
 \multirow{2}{*}{Method} & sup. train. & self sup. train. & \multirow{2}{*}{PSNR$\uparrow$} & \multirow{2}{*}{SSIM$\uparrow$}   \\ %\rowcolor{tableHeadGray}
 &on GoPro&on HighREV&&\\
 
 \hline \hline
EDI~\cite{edi_pan}             & \xmark   & \cmark        & 25.32            & 0.753 \\
% SRN~\cite{tao2018scale}        & \xmark           & -                & -       \\
SRN+~\cite{tao2018scale}       & \cmark   & \xmark        & 25.65            & 0.836  \\
% HINet~\cite{chen2021hinet}     & \xmark           & -                & -       \\
HINet+~\cite{chen2021hinet}    & \cmark   & \xmark        & 28.70            & 0.910    \\
EFNet~\cite{sun2022event}      & \cmark   & \xmark        & 29.55            & 0.936   \\
REFID~\cite{sun2023event}      & \cmark   & \xmark        & 28.97            & 0.894  \\
Ours                           & \cmark   & \xmark        & 28.72            & 0.910 \\
Ours                           & \xmark   & \cmark        & 30.04            & 0.931 \\
\textbf{Ours}                   & \cmark   & \cmark        & 32.70            & 0.951  \\
% \bottomrule
\hline
\end{tabular}
}
\label{table:highrev}
}
}
\end{table}

==> tables/gopro_results.tex <==
\begin{minipage}[t]{0.48\linewidth}
% \captionsetup{font=small}
\captionof{table}{\small \textbf{Comparison of motion deblurring methods on the GoPro dataset~\cite{nah2017deep}.} SRN+ and HINet+ denote event-enhanced versions of SRN~\cite{tao2018scale} and HINet~\cite{chen2021hinet}.}
% \vspace{-3mm}
\centering
\small
% \tiny
\resizebox{1\textwidth}{!}{
%\setlength{\tabcolsep}{30pt}     % adjust the width of cell
\renewcommand\arraystretch{1.0} % adjust hight of the row
\begin{tabular}{ l  || c | c |  c  |  c  }
\bottomrule[0.15em]
\rowcolor{tableHeadGray}
 Method &  Self-Sup.  &Events & PSNR $\uparrow$ & SSIM $\uparrow$  \\ \hline \hline
EDI~\cite{edi_pan}                  &\cmark&\cmark& 27.34 & 0.901 \\
Nah \etal \cite{nah2017deep}        &\xmark&\xmark& 29.08 & 0.914 \\
SRN~\cite{tao2018scale}             &\xmark&\xmark& 30.26 & 0.934 \\
SRN+~\cite{tao2018scale}            &\xmark&\cmark& 31.02 & 0.936 \\
D$^{2}$Nets~\cite{shang2021bringing}&\xmark&\cmark& 31.60 & 0.940 \\
LEMD~\cite{jiang2020}               &\xmark&\cmark& 31.79 & 0.949 \\
HINet~\cite{chen2021hinet}          &\xmark&\xmark& 32.71 & 0.959 \\
Restormer~\cite{Zamir2021Restormer} &\xmark&\xmark& 32.92 & 0.961 \\
ERDNet~\cite{haoyu2020learning}     &\xmark&\cmark& 32.99 & 0.935 \\
HINet+~\cite{chen2021hinet}         &\xmark&\cmark& 33.69 & 0.961 \\
EFNet~\cite{sun2022event}           &\xmark&\cmark& 35.46 & 0.972 \\
REFID~\cite{sun2023event}           &\xmark&\cmark& \textbf{35.91} & \textbf{0.973}\\ \hline \textbf{Ours}                &\cmark&\cmark& 28.88 & 0.912 \\
\textbf{Ours}                       &\xmark&\cmark& 35.52 & 0.972 \\
\bottomrule
\hline
\end{tabular}
}
\label{table:gopro}
% \vspace{-0.5cm}
\end{minipage}

==> tables/highrev_results.tex <==
\begin{minipage}[t]{0.49\linewidth}
    \centering
\small
\captionof{table}{\small \textbf{Comparison of event-based motion deblurring methods on the HighREV dataset~\cite{sun2023event}.} Methods with a + denote event-enhanced versions.}
\resizebox{1\textwidth}{!}{
%\setlength{\tabcolsep}{20pt}     % adjust the width of cell
\renewcommand\arraystretch{1.0} % adjust hight of the row
\begin{tabular}{ l  || c |  c  |  c |  c }
\bottomrule[0.15em]
\rowcolor{tableHeadGray}
  & sup. train. & self sup. train. &  & \\ %\rowcolor{tableHeadGray}
 \rowcolor{tableHeadGray}
 \multirow{-2}{*}{Method}&on GoPro&on HighREV&\multirow{-2}{*}{PSNR$\uparrow$}&\multirow{-2}{*}{SSIM$\uparrow$}\\
 
 \hline \hline
EDI~\cite{edi_pan}             & \xmark   & \cmark        & 25.32            & 0.753 \\
% SRN~\cite{tao2018scale}        & \xmark           & -                & -       \\
SRN+~\cite{tao2018scale}       & \cmark   & \xmark        & 25.65            & 0.836  \\
% HINet~\cite{chen2021hinet}     & \xmark           & -                & -       \\
HINet+~\cite{chen2021hinet}    & \cmark   & \xmark        & 28.70            & 0.910    \\
EFNet~\cite{sun2022event}      & \cmark   & \xmark        & 29.55            & 0.936   \\
REFID~\cite{sun2023event}      & \cmark   & \xmark        & 28.97            & 0.894  \\\hline
\textbf{Ours}                           & \cmark   & \xmark        & 28.72            & 0.910 \\
\textbf{Ours}                           & \xmark   & \cmark        & 30.04            & 0.931 \\
\textbf{Ours}                   & \cmark   & \cmark        & 32.70            & 0.951  \\
% \bottomrule
\bottomrule
\end{tabular}
}
\label{table:highrev}
%\vspace{0.5cm}
\end{minipage}
\hfill
